Resilient Active Information Gathering with Mobile Robots

Applications of safety, security, and rescue in robotics, such as multi-robot target tracking, involve the execution of information acquisition tasks by teams of mobile robots. However, in failure-prone or adversarial environments, robots get attacked, their communication channels get jammed, and their sensors may fail, resulting in the withdrawal of robots from the collective task, and consequently the inability of the remaining active robots to coordinate with each other. As a result, traditional design paradigms become insufficient and, in contrast, resilient designs against system-wide failures and attacks become important. In general, resilient design problems are hard, and even though they often involve objective functions that are monotone or submodular, scalable approximation algorithms for their solution have been hitherto unknown. In this paper, we provide the first algorithm, enabling the following capabilities: minimal communication, i.e., the algorithm is executed by the robots based only on minimal communication between them; system-wide resiliency, i.e., the algorithm is valid for any number of denial-of-service attacks and failures; and provable approximation performance, i.e., the algorithm ensures for all monotone (and not necessarily submodular) objective functions a solution that is finitely close to the optimal. We quantify our algorithm's approximation performance using a notion of curvature for monotone set functions. We support our theoretical analyses with simulated and real-world experiments, by considering an active information gathering scenario, namely, multi-robot target tracking.

==> tex/SectionII_edited_by_Brent.tex <==
\section{Problem Formulation}\label{sec:prob_form}
%(purpose of this section)
We formalize the resilient active information acquisition problem considered in this paper.
%(brief description of the problem in hand)
%In particular, the problem of  \textit{(non-resilient)} active information acquisition suggests tracking the evolution of a phenomenon (target phenomenon) by (i)~using sensors mounted on a team of mobile robots, and~(ii)~planning the robots' motion (control policy) to optimize the team's collective tracking capability of the phenomenon (with respect to an information acquisition metric).  Correspondingly, in this paper, the problem of  \textit{resilient} active information acquisition aims to ensure the success of the aforementioned collective task despite (i)~failures or denial-of-service attacks that cause the withdrawal of robots from the collective task, and, sequentially,~(ii)~failures or denial-of-service attacks to the robot's communication network that prevents the remaining (active) robots from collectively re-planning their coordinated motion.
To begin, the problem of \textit{(non-resilient)} active information acquisition is to track the evolution of a phenomenon (target phenomenon) by designing control policies for a team of mobile sensing robots to track the evolution of a phenomenon of interest (target phenomenon) subject to robot motion constraints, a target evolution model, and the observation model of the sensors. In this paper, we address the problem of \textit{resilient} active information acquisition which is to enable the success of the collective information gathering task despite failures or denial-of-service attacks that cause the withdrawal of robots from the collective task. This removal of robots from the collective results in disruption to the robot's communication network and prevents the remaining (active) robots from jointly re-planning their coordinated motion.
\subsection{Definitions}
%\subsection{Target phenomenon, robots, sensors, control policies, information acquisition metrics, and communication network} 
\label{sec:definitions}

%purpose of this section
%Towards the definition of the problem of resilient active information acquisition considered in this paper, we introduce in the following paragraphs standard models for the notions of \textit{target phenomenon}, \textit{robots}, \textit{sensors}, \textit{control policies}, and \textit{information acquisition metric}, as well as, standard assumptions on the inter-robot \emph{communication network}.

\setcounter{paragraph}{0}

\paragraph{Robots}
%why this notion is important in our problem  
The task of the information acquisition problem is to design control policies for sensors mounted on mobile robots. We begin by defining the motion model for the robots. Let $\calV$ denote the set of available robots, i.e. each index $i\in\calV$ uniquely identifies a robot in the team. We model the robot's dynamics as a discrete time general non-linear system:
\begin{align}\label{eq:robot}
x_{i,t} = f_i(x_{i,t-1},u_{i,t-1}),~~~i \in \calV,~~~t=1,2,\ldots,T,
\end{align}
where the state of the $i$th robot at time $t$ is $x_{i,t} \in \mathbb{R}^{n_{x_{i,t}}}$. The vector $u_{i,t} \in \calU_{i,t}$ represents the control input, where the set of possible control actions  $\calU \subseteq \mathbb{R}^{m_{i,t}}$ is a \textit{finite} set of admissible inputs.
\b{Can we get rid of the time horizon here? I think it is not necessary for describing the models, but instead for the objective function}
%Active information acquisition suggests to track the evolution of the target phenomenon in eq.~\eqref{eq:target} by using sensors mounted on mobile robots.  In this paper, we~denote the set of available robots as~$\calV$ (that is, $\calV$ is a set of indices such that each index $i\in\calV$ uniquely identifies a robot in the team), and model each robot's dynamics as a standard discrete-time (possibly) non-linear system:
%description of notion

\paragraph{Target phenomenon}  
%why this notion is important in our problem (how it participates in the our problem) 
The objective of the information acquisition task is to estimate the target phenomenon. In this work, we model the phenomenon's evolution as a standard discrete-time (possibly time-varying) linear system with additive Gaussian process noise:
%description of notion
\begin{align}\label{eq:target}
y_{t} = A_{t-1} y_{t-1} + w_{t-1},~~~t=1,2,\ldots,T,
\end{align}
where the vector $y_t \in \mathbb{R}^{n_{y_t}}$ represents the state of the phenomenon at time~$t$, the vector $w_t \in \mathbb{R}^{n_{y_{t+1}}}$ represents process noise, the matrix $A_t$ has suitable dimension, and the number~$T$ represents a finite (time) horizon. In~addition, we~consider the initial condition~$y_0$ to be a Gaussian random variable with covariance~$\Sigma\att{0}{0}$, and the process noise $w_t$ to be a Gaussian random variable with mean zero and covariance $W_t$, such that $w_t$ is independent of $y_1$ and $w_{t'}$, for all $t'=1,2,\ldots,T$, $t'\neq t$.

\paragraph{Sensors}
%why this notion is important in our problem 
%In this paper, the active information acquisition over the target phenomenon in eq.~\eqref{eq:target} is enabled by sensors mounted on the mobile team of robots in eq.~\eqref{eq:robot}. 
At each time  the mounted sensors produce measurements dependent on the state of both the phenomenon and the robot that the sensor is mounted to; in this paper, we consider the sensor measurements to be linearly dependent on the state of the target phenomenon (this standard modeling consideration is without loss of generality whenever linearization over the current estimate of the phenomenon's state is possible), and (possibly) non-linearly \mbox{dependent on the robots' state, as follows:}
%description of notion
\begin{align}\label{eq:sensors}
z_{i,t}=H_{i,t}(x_{i,t})y_{i,t}+v_{i,t}(x_{i,t}),~~~i\in\calV,~~~t=1,2,\ldots,T,
\end{align}
where the vector $z_{i,t} \in \mathbb{R}^{n_{z_{i,t}}}$ is the measurement obtained  at time $t$ by the on-board sensor at robot $i$, the vector  $v_{i,t}(x_{i,t})\in \mathbb{R}^{n_{z_{i,t}}}$ represents measurement noise, and the matrix $H_{i,t}(x_{i,t})$ has suitable dimension. In~addition, we~consider the noise $v_{i,t}(x_{i,t})$ to be a Gaussian random variable with mean zero and covariance $V_{i,t}(x_{i,t})$, such that~$v_{i,t}(x_{i,t})$ is independent of the phenomenon's initial condition $y_1$, of the phenomenon's process noise $w_{t'}$, for any $t'\neq t$, as well as, of the noises $v_{i',t'}$, for all $t'\neq t$, and any $i'\in\calV$, $i' \neq i$.

\paragraph{Control policies}
%why this notion is important in our problem 
The objective of active information acquisition, that is, to track the evolution of the target phenomenon in eq.~\eqref{eq:target}, is achieved by selecting the motion plan (control policy) of each robot in eq.~\eqref{eq:robot} such that the robots' collective sensing capability (from the on-board sensors) is optimized.  Generally, each robot selects its motion plan by having access to different levels of information (e.g., only the measurements collected by its on-board sensors or also the measurements collected by its neighbouring robots).  Herein, we are interested in information acquisition with minimal communication between the robots during the execution of the information acquisition task and, as a result, we consider each robot to decide its control policy based on merely the measurements collected by its on-board sensors; that is:
%description of notion
\begin{equation}\label{eq:control_policies}
u_{i,t} = u_{i,t}(z_{i,1}, z_{i,2}, \ldots, z_{i,t}),~~~i\in \calV,~~~t = 1,2,\ldots,T.
\end{equation}
Control policies of the form in eq.~\eqref{eq:control_policies} are called \emph{admissible}. 

\paragraph{Information acquisition metric} 
The problem of active information acquisition suggests the team of robots in $\calV$ to select their admissible control policies, namely,
\begin{equation}
u_{1:T}\triangleq \{u_{i,t}(z_{i,1}, z_{i,2}, \ldots, z_{i,t}): i \in \calV,~~~t=1,2,\ldots,T\}, \label{def:uTcalV}
\end{equation}
to maximize the team's tracking capability of the evolution of the target phenomenon in eq.~\eqref{eq:target}.  In more detail, the team's tracking capability is quantified by an information acquisition metric, denoted, henceforth, by~$\metric$.
Naturally, the metric $\metric$ is a (real-valued) function that depends on the robots' control policies, and on both the target phenomenon's initial condition $y_0$ and the robots' initial conditions $\{x_{i,0}:i\in \calV\}$; i.e.,
\begin{equation}\label{eq:metric}
\metric=\metric(u_{1:T}),
\end{equation}
where $u_{1:T}$ is defined in eq.~\eqref{def:uTcalV}, and where, for notational simplicity, we suppress the dependence of $\metric$ on the initial conditions $y_0$ and $\{x_{i,0}:i\in \calV\}$.
Standard examples of information acquisition metrics of the same form as $\metric$'s include the mutual information $I(y_{T}; z_{1:T})$, the conditional entropy $H(y_{T}| z_{1:T})$, and the average minimum mean square error $M(y_{1:T}, z_{1:T})$ across all times $t=1,2,\ldots,T$, wherein we let $ z_{1:T}\triangleq \{z_{i,t}:i\in \calV,~~~t=1,2,\ldots,T\}$, i.e., $z_{1:T}$ is the set of measurements collected by all robots' across all times, and, similarly, $y_{1:T}\triangleq\{y_1,y_2,\ldots,y_T\}$ (see~\cite{atanasov2015decentralized,atanasov2014information,tzoumas2017sensing}, and the references therein, both for more details and for more examples of metrics of the same form as $\metric$'s).

\paragraph{Communication network} For the robots in $\calV$ to collectively achieve their objective of active information acquisition, they need to coordinate their motion, and, as a result, they need to (possibly) share their control policies at each time $t=1,2,\ldots,T$\!.  In this paper, we consider an inter-robot communication network that is \textit{connected} and \textit{decentralized}, i.e., when no attacks and failures affect the communication network, for each two robots $i,j\in\calV$, there exist a path of communication between them: that is, there exist robots $r_1,r_2,\ldots, r_p \in\calV$ (for some integer $0\leq p < |\calV|$; when $p=0$, then $i$ and $j$ are neighbours, and can communicate directly)  such that robot $i$ can communicate with robot $r_1$, then for each $k=1,2,\ldots, p-1$, robot $r_k$ can communicate with robot $r_{k+1}$, and robot $r_p$ can communicate with robot~$j$.

\subsection{Resilient Active Information Acquisition} 
\label{sec:problem_definition}

%(purpose of section)
In this paper, the problem of \textit{resilient} active information acquisition aims to ensure that an active information acquisition task performed by a team of robots remains successful despite (i)~failures or denial-of-service attacks that cause the withdrawal of robots from the collective task, and, sequentially,~(ii)~failures or denial-of-service attacks to the robot's communication network that prevents the remaining (active) robots from collectively re-planning their coordinated motion.  We formalize next the definition of an \emph{active robot set}, and, then, that of \emph{resilient active information acquisition}.

%(motivates following definitions on active control policies)
\begin{mydef}[Active robot set, and active control policies]\label{def:active_set}
Consider an information acquisition task, and a set of robots~$\calV$ that can be (possibly) used to complete the task over a time horizon $T$; if only the subset of robots $\calR\subseteq \calV$ participates in the completion of the information acquisition task (and the robots in $\calV\setminus \calR$ never participate), then we say (i)~that the subset of robots $\calR\subseteq \calV$ is an \emph{active robot set}, and~(ii)~that the corresponding sets of admissible control policies:
\begin{equation}
\cp{t}{\calR}\triangleq \{u_{i,t}(z_{i,1}, z_{i,2}, \ldots, z_{i,t}): i \in \calR\},~~~ t=1,2,\ldots,T,\label{eq:active_control_policies}
\end{equation}
are the \emph{active control policies}, per eq.~\eqref{eq:control_policies}.
\end{mydef}

We define next the main problem in this paper.

%(problem definition)
\begin{myproblem}
[Resilient Active Information Acquisition]
\label{pr:resil_active_inf_acq}
%\emph{\textbf{(Resilient Active Information Acquisition)}}
Given a time horizon~$T$, consider a target phenomenon per eq.~\eqref{eq:target}; in addition, consider a set of robots $\calV$, with dynamics per eq.~\eqref{eq:robot}, with sensing capabilities per eq.~\eqref{eq:sensors}, and with admissible control policies per eq.~\eqref{eq:control_policies}; moreover, consider an information acquisition metric $\metric$ per eq.~\eqref{eq:metric}; finally, consider a number $a \leq |\calV|$, that represents the maximum number of possible robot withdrawals from $\calV$, e.g., due to failures or attacks, which (in the worst-case) happen in the beginning of time. Then, for all robots $i\in\calV$, and for all times $t=1,2,\ldots,T$, find admissible control policies $u_{i,t}$ to maximize metric $g$ against a \emph{worst-case} withdrawal from $\calV$ of a subset of robots $\calA\subseteq\cal \calV$, with cardinality at most~$a$:
\begin{align}\label{preq:resil_active_inf_acq}
\begin{split}
&\hspace*{-17mm}\max_{\scriptsize\begin{array}{c}
u_{i,t} \in \mathbb{U}_{i,t},i\in\calV,\\
 t=1,2\ldots,T
\end{array}}\min_{\calA\subseteq \calV} \;\;\;\metric(\cp{1:T}{\calV\setminus \calA}):\\
&\hspace*{-3mm}\text{such that, for all } i\in\calV,~~~t=1,2,\ldots,T:\\
&\;y_{t} = A_{t-1} y_{t-1} + w_{t-1},\\
&\;x_{i,t} = f_i(x_{i,t-1},u_{i,t-1}),\\
&\;z_{i,t}=H_{i,t}(x_{i,t})y_{i,t}+v_{i,t}(x_{i,t}),\\
&\;u_{i,t}=u_{i,t}(z_{i,1}, z_{i,2}, \ldots, z_{i,t}),\\
&\;|\calA|\leq a,
\end{split}
\end{align}
where $\cp{1:T}{\calV\setminus \calA}\triangleq \{\cp{t}{\calV\setminus \calA}: t =1,2,\ldots,T\}$, per eq.~\eqref{eq:active_control_policies}, and $y_{1:T}\triangleq\{y_t: t=1,2,\ldots,T\}$.
\end{myproblem}

%(interpretation of above problem:
%(i) What was the old paradigm)
%(ii) What the new paradigm calls for)
Problem~\ref{pr:resil_active_inf_acq} goes beyond the objective of active information acquisition, where the motion of a team of robots is pre-planned to optimize the robots' tracking capability of a target phenomenon over a time horizon, by accounting in the motion pre-planning for worst-case failures and attacks that (i)~not only may cause the withdrawal of robots from the information acquisition task, at the very beginning of the (observation) time horizon, but also, (ii)~they may prevent the remaining active robots from collectively re-planning their motion, e.g., by jamming the inter-robot communication capabilities. 

%(Conclusion of section:) 
In the following sections, we provide the first scalable algorithm for Problem~\ref{pr:resil_active_inf_acq}, that also enables the decentralized solution of Problem~\ref{pr:resil_active_inf_acq}, along with provable approximation performance guarantees.  In particular, we make our contributions with respect to information acquisition metrics that belong to the class of monotone and (approximately) submodular functions in the active robot set; notably, the~aforementioned class of functions captures standard metrics in the literature of information acquisition, such as the mutual information $I(y_{T}; z_{1:T})$, the conditional entropy $H(y_{T}| z_{1:T})$, and the average minimum mean square error $M(y_{1:T}, z_{1:T})$ across all times $t=1,2,\ldots,T$ (see~\cite{atanasov2014information,atanasov2015decentralized,tzoumas2017sensing}, respectively).



==> tex/preamble_packages.tex <==
%!TEX root = main.tex

% LC: debug
%==========================================================================
%\usepackage{refcheck}
%\usepackage[notref]{showkeys}
%==========================================================================

% LC: to be used for TRO
%==========================================================================
% \usepackage{mathptmx} % assumes new font selection scheme installed
%\usepackage{times} % assumes new font selection scheme installed
%==========================================================================
\usepackage{comment}
\usepackage{siunitx}
\usepackage{relsize}
\usepackage{ifthen}

\usepackage[caption=false]{subfig}

% \begin{comment}
% % Fancy formatting 
% \usepackage[tracking=false,kerning=true,spacing=true]{microtype}
% \usepackage[caption=false]{subfig}

% \usepackage[style=numeric-comp,sorting=none,firstinits=true, maxnames=3,bibstyle=numeric,abbreviate=false,defernums=true,eprint=false,backend=bibtex]{biblatex}
% \renewcommand{\bibfont}{\footnotesize}
% % \DeclareFieldFormat[article]{pages}{#1}%
% % \DeclareFieldFormat[inproceedings]{pages}{#1}%

% \AtEveryBibitem{%
%   \ifentrytype{article}{%
%     \clearfield{pages}%
%   }{%
%   }%
%   \ifentrytype{inproceedings}{%
%     \clearfield{pages}%
%   }{%
%   }%
% }
% \end{comment}

% \bibliography{commons/bib/strings_long}
% \bibliography{commons/bib/all_only_one_w_pages}
% \bibliography{../../references/references}

% \usepackage[noadjust]{cite}
%\usepackage[vlined,ruled,linesnumbered]{algcompatible}
\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{rotating}
\usepackage{color}
\usepackage{enumerate}
\usepackage[T1]{fontenc}
\usepackage{psfrag}
\usepackage{epsfig} % for postscript graphics files
%\usepackage{subfigure}
% \usepackage{hyperref}
\usepackage{booktabs}
\usepackage{graphicx,url}
\usepackage{multirow}
\usepackage{array}
\usepackage{latexsym}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{amsthm}
\usepackage{xstring}
%\usepackage[noend]{algorithmic}
\usepackage{multirow}
\usepackage{xcolor}
\usepackage{prettyref}
\usepackage{flexisym}
\usepackage{bigdelim}
\usepackage{breqn} % load this last
\usepackage{listings}
\let\labelindent\relax
\usepackage{enumitem}
\usepackage{xspace}
\usepackage{bm}
\graphicspath{{./figures/}}
\usepackage{tikz}
\usetikzlibrary{matrix,calc}


%\usepackage{amsthm} % math
\usepackage{lineno}



%\usepackage{ifpdf}
% Heiko Oberdiek's ifpdf.sty is very useful if you need conditional
% compilation based on whether the output is pdf or dvi.
% usage:
% \ifpdf
%   % pdf code
% \else
%    dvi code
% \fi
% The latest version of ifpdf.sty can be obtained from:
% http://www.ctan.org/tex-archive/macros/latex/contrib/oberdiek/
% Also, note that IEEEtran.cls V1.7 and later provides a builtin
% \ifCLASSINFOpdf conditional that works the same way.
% When switching from latex to pdflatex and vice-versa, the compiler may
% have to be run twice to clear warning/error messages.

% *** GRAPHICS RELATED PACKAGES ***
%
%\ifCLASSINFOpdf
  % \usepackage[pdftex]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../pdf/}{../jpeg/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
%\else
  % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
  % will default to the driver specified in the system graphics.cfg if no
  % driver is specified.
  % \usepackage[dvips]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../eps/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.eps}
%\fi


\usepackage{mdwlist}
\let\stditemize\itemize
\let\endstditemize\enditemize
\let\itemize\undefined
\makecompactlist{itemize}{stditemize}

%\let\stdenumerate\enumerate
%\let\endstdenumerate\endenumerate
%\let\enumerate\undefined
%\makecompactlist{enumerate}{stdenumerate}
 

